Towards a background-free neutrinoless double beta decay experiment based on a fluorescent bicolor sensor

Searching for neutrinoless double beta decays ($\beta\beta0\nu$) is the only practical way to establish if the neutrinos are their own antiparticles. Due to the smallness of neutrino masses, the lifetime of $\beta\beta0\nu$ is expected to be at least ten orders of magnitude smaller than the noise associated with the natural radioactive chains. A positive identification of $\beta\beta0\nu$ decays requires, ultimately, finding a signal that cannot be mimicked by radioactive backgrounds. This signal could be the observation of the daughter atom in the decay, since no known background processes induce a Z+2 transformation. In particular, the $\beta\beta0\nu$ decay of Xe-136 could be established by detecting the doubly ionised daughter atom, Ba$^{2+}$. Such a detection could be achieved via a sensor made of a monolayer of molecular indicators. The Ba$^{2+}$ would be captured by one of the molecules in the sensor, and the presence of the single chelated indicator would be subsequently revealed by a strong fluorescent response from repeated interrogation with a laser system. Here we describe a fluorescent bicolor indicator that binds strongly to Ba$^{2+}$ and shines very brightly, shifting its emission colour from green to blue when chelated in dry medium, thus allowing the unambiguous identification of single barium atoms in the sensor, and permitting a positive identification of the $\beta\beta0\nu$ decay of Xe-136 in a gas chamber, that could led to a background-free experiment.

==> abstract.tex <==
\abstract{
Neutrinoless double beta decay (\bbonu) is a putative nuclear decay that can occur if, and only if, neutrinos are their own antiparticles. Due to the smallness of neutrino masses, the lifetime of \bbonu\ is expected to be larger than \SI{1E+26}{\yr}, and any putative signal will be many orders of magnitude smaller than the backgrounds associated with the natural radioactive chains. Future experiments will require the development of new experimental techniques to suppress those backgrounds. Since only \bbonu\ converts xenon to barium, detection of the daughter ion in candidate decay events effectively eliminates backgrounds. It has been recently proposed that a xenon gas time projection chamber could unambiguously tag the \bbonu\ decay 
$\XE \rightarrow \Bapp + 2e^- (+2 \nu)$ by detecting the resulting \Bapp\ ion in a single-atom sensor made of a monolayer of molecular indicators. The \Bapp\ would be captured by one of the molecules in the sensor, and the presence of the single chelated indicator would be subsequently revealed by a strong fluorescent response from repeated interrogation with a suitable laser system. 
Here we describe a fluorescent bicolor indicator that binds strongly to \Bapp\ 
and shines very brightly, shifting its emission colour from green to blue when chelated in dry medium, thus providing a discrimination factor with respect to the unchelated species in excess of $10^4$.
%, three orders of magnitude larger than that found with existing indicators. 
This allow us to demonstrate the feasibility of a new sensor for \Bapp\ tagging based on a monolayer of this bicolor indicator and two-photon absorption microscopy. Such a sensor could be the basis of a background-free \bbonu\ experiment.}

